VISTA: Monocular Segmentation-Based Mapping for Appearance and View-Invariant Global Localization

Global localization is critical for autonomous navigation, particularly in scenarios where an agent must localize within a map generated in a different session or by another agent, as agents often have no prior knowledge about the correlation between reference frames. However, this task remains challenging in unstructured environments due to appearance changes induced by viewpoint variation, seasonal changes, spatial aliasing, and occlusions -- known failure modes for traditional place recognition methods. To address these challenges, we propose VISTA (View-Invariant Segmentation-Based Tracking for Frame Alignment), a novel open-set, monocular global localization framework that combines: 1) a front-end, object-based, segmentation and tracking pipeline, followed by 2) a submap correspondence search, which exploits geometric consistencies between environment maps to align vehicle reference frames. VISTA enables consistent localization across diverse camera viewpoints and seasonal changes, without requiring any domain-specific training or finetuning. We evaluate VISTA on seasonal and oblique-angle aerial datasets, achieving up to a 69% improvement in recall over baseline methods. Furthermore, we maintain a compact object-based map that is only 0.6% the size of the most memory-conservative baseline, making our approach capable of real-time implementation on resource-constrained platforms.

==> archive.tex <==
    \item Developed an auto-segmentation tracking pipeline to recreate sparse 3D environment maps from monocular RGB imagery, which utilizes SAM \cite{kirillov2023segment} to produce object masks used to prompt SAM2 \cite{ravi2024sam2segmentimages} for robust object tracking. This object-based monocular tracking allows for sparse 3D environment reconstruction, containing object locations and their respective uncertainties, accurate enough for efficient and reliable global localization.
    \item A geometric submap correspondence search method that performs data associations 74x faster than the average match time of the baseline approaches and scales according to number of submaps rather than number of keyframes in contrast to the learning-based data association methods.
    \item Evaluation of our proposed method on challenging indoor, unstructured datasets, achieving 74\% higher maximum precision compared to both traditional and learning-based visual place recognition (VPR) baseline methods, with a map over 1500x smaller than the average baseline map size. We demonstrate that our approach achieves global localization by resolving geometric ambiguity between submaps, regardless of viewpoint variation, visual feature changes, perceptual aliasing, motion blur, and partial occlusions.
